Towards Malware Detection via CPU Power Consumption: Data Collection Design and Analytics (Extended Version)

This paper presents an experimental design and data analytics approach aimed at power-based malware detection on general-purpose computers. Leveraging the fact that malware executions must consume power, we explore the postulate that malware can be accurately detected via power data analytics. Our experimental design and implementation allow for programmatic collection of CPU power profiles for fixed tasks during uninfected and infected states using five different rootkits. To characterize the power consumption profiles, we use both simple statistical and novel, sophisticated features. We test a one-class anomaly detection ensemble (that baselines non-infected power profiles) and several kernel-based SVM classifiers (that train on both uninfected and infected profiles) in detecting previously unseen malware and clean profiles. The anomaly detection system exhibits perfect detection when using all features and tasks, with smaller false detection rate than the supervised classifiers. The primary contribution is the proof of concept that baselining power of fixed tasks can provide accurate detection of rootkits. Moreover, our treatment presents engineering hurdles needed for experimentation and allows analysis of each statistical feature individually. This work appears to be the first step towards a viable power-based detection capability for general-purpose computers, and presents next steps toward this goal.

==> 001-recommended-packages.tex <==

%cmap has to be loaded before any font package (such as cfr-lm)
\usepackage{cmap}
\usepackage[T1]{fontenc}

\usepackage{graphicx}

%Even though `american`, `english` and `USenglish` are synonyms for babel package (according to https://tex.stackexchange.com/questions/12775/babel-english-american-usenglish), the llncs document class is prepared to avoid the overriding of certain names (such as "Abstract." -> "Abstract" or "Fig." -> "Figure") when using `english`, but not when using the other 2.
%english has to go last to set it as default language
\usepackage[ngerman,english]{babel}
%Hint by http://tex.stackexchange.com/a/321066/9075 -> enable "= as dashes
\addto\extrasenglish{\languageshorthands{ngerman}\useshorthands{"}}

%better font, similar to the default springer font
%cfr-lm is preferred over lmodern. Reasoning at http://tex.stackexchange.com/a/247543/9075
\usepackage[%
rm={oldstyle=false,proportional=true},%
sf={oldstyle=false,proportional=true},%
tt={oldstyle=false,proportional=true,variable=true},%
qt=false%
]{cfr-lm}
%
%if more space is needed, exchange cfr-lm by mathptmx
%\usepackage{mathptmx}

%for demonstration purposes only
\usepackage[math]{blindtext}

%Sorts the citations in the brackets
%It also allows \cite{refa, refb}. Otherwise, the document does not compile.
%  Error message: "White space in argument"
\usepackage{cite}


%% If you need packages for other papers,
%% START COPYING HERE
%% COPY ALSO cmap and fontenc from lines 10 to 12

%extended enumerate, such as \begin{compactenum}
\usepackage{paralist}

%put figures inside a text
%\usepackage{picins}
%use
%\piccaptioninside
%\piccaption{...}
%\parpic[r]{\includegraphics ...}
%Text...

%for easy quotations: \enquote{text}
\usepackage{csquotes}

%enable margin kerning
\usepackage{microtype}

%tweak \url{...}
\usepackage{url}
%\urlstyle{same}
%improve wrapping of URLs - hint by http://tex.stackexchange.com/a/10419/9075
\makeatletter
\g@addto@macro{\UrlBreaks}{\UrlOrds}
\makeatother
%nicer // - solution by http://tex.stackexchange.com/a/98470/9075
%DO NOT ACTIVATE -> prevents line breaks
%\makeatletter
%\def\Url@twoslashes{\mathchar`\/\@ifnextchar/{\kern-.2em}{}}
%\g@addto@macro\UrlSpecials{\do\/{\Url@twoslashes}}
%\makeatother

%diagonal lines in a table - http://tex.stackexchange.com/questions/17745/diagonal-lines-in-table-cell
%slashbox is not available in texlive (due to licensing) and also gives bad results. This, we use diagbox
%\usepackage{diagbox}

%required for pdfcomment later
\usepackage{xcolor}


%enable nice comments
%this also loads hyperref
\usepackage{pdfcomment}

%enable hyperref without colors and without bookmarks
% \hypersetup{hidelinks,
%   colorlinks=true,
%   allcolors=black,
%   pdfstartview=Fit,
%   breaklinks=true}

%enables correct jumping to figures when referencing
% \usepackage[all]{hypcap}

% \newcommand{\commentontext}[2]{\colorbox{yellow!60}{#1}\pdfcomment[color={0.234 0.867 0.211},hoffset=-6pt,voffset=10pt,opacity=0.5]{#2}}
% \newcommand{\commentatside}[1]{\pdfcomment[color={0.045 0.278 0.643},icon=Note]{#1}}

%compatibality with packages todo, easy-todo, todonotes
% \newcommand{\todo}[1]{\commentatside{#1}}
% %compatiblity with package fixmetodonotes
% \newcommand{\TODO}[1]{\commentatside{#1}}

%enable \cref{...} and \Cref{...} instead of \ref: Type of reference included in the link
\usepackage[capitalise,nameinlink]{cleveref}
%Nice formats for \cref
% \crefname{section}{Sect.}{Sect.}
% \Crefname{section}{Section}{Sections}

\usepackage{xspace}
%\newcommand{\eg}{e.\,g.\xspace}
%\newcommand{\ie}{i.\,e.\xspace}
\newcommand{\eg}{e.\,g.,\ }
\newcommand{\ie}{i.\,e.,\ }

%introduce \powerset - hint by http://matheplanet.com/matheplanet/nuke/html/viewtopic.php?topic=136492&post_id=997377
% \DeclareFontFamily{U}{MnSymbolC}{}
% \DeclareSymbolFont{MnSyC}{U}{MnSymbolC}{m}{n}
% \DeclareFontShape{U}{MnSymbolC}{m}{n}{
%     <-6>  MnSymbolC5
%   <6-7>  MnSymbolC6
%   <7-8>  MnSymbolC7
%   <8-9>  MnSymbolC8
%   <9-10> MnSymbolC9
%   <10-12> MnSymbolC10
%   <12->   MnSymbolC12%
% }{}
% \DeclareMathSymbol{\powerset}{\mathord}{MnSyC}{180}


%% END COPYING HERE

==> 04-bottom-matter.tex <==
%% keywords
\begin{keywords}
malware, power model, intrusion detection, anomaly detection
\end{keywords}

==> 3-experiment-2.tex <==
\section{Test Bed Design, Rootkits, \& Data Collection}
\label{sec:expDesignDataColl}
%The goal of our experiments is to detect the presence of rootkits when a set of repeatable tasks are executed on the general-purpose computer.
Our conjecture is that for a fixed task, malware's actions will produce sufficient deviation in the power profile to admit detection.
To test this, we use three tasks, two tasks that we believe will change in the presence of rootkits\textemdash web browsing with Internet Explorer (IE) and probing the registry\textemdash and a final task, letting the computer sit idle, to test if malware executions are detectable when no other execution commands are given.
IE was chosen because it has been proven that some rootkits affect the performance of browsers~\cite{118}.
The registry was chosen because rootkits often make modifications to it and then use a driver to hide the modified registry keys from observation~\cite{Hoglund08}.
Registry modification is a common element of most Windows programs, so merely watching process behavior for this trait would not give accurate malware detection.
What is uncommon is for programs to then take actions that prevent their registry modifications from being observed by other processes scanning the registry, a concealing characteristic of some malware~\cite{Hoglund08}.

%Next we discuss the hardware and software configuration used for the experiments, how the power data was collected, and the rootkits used to produce our data.

\subsection{Hardware and Software Configuration}
Anticipating that the effects of malware execution on power signals are subtle, significant effort was spent  sensing and recording the power use data.  %{\color{magenta} We go into some detail in this section to describe how we converged on a successful design that records the power use signals for a general-purpose computer, so that they could be segmented and compared across different experiments.}
% The algorithms used to detect malware rely heavily on being comparison of data from different experiments.
Our experiments were run on a Dell OptiPlex 755 machine running 32-bit Windows 7.
To record the data for our experiments, we used a Measurement Computing Data Acquisition\footnote{DAQ model USB-1608G Series with 16 channels used.  \url{www.mccdaq.com}}
(DAQ) system.
Separate channels on the DAQ were connected through a printed circuit board (PCB) sensor to separate voltage sources on the computer's motherboard power connector, and the voltage and current were collected  on each DC power channel.
%More details about the hardware configuration can be found here~\cite{hernandez2017}.

%{\color{magenta} Initially we were monitoring a total of 11 DC power channels from the ATX-standard power supply. From those 11 channels, four pins had a signal of +3.3V, five pins had a signal of +5V, and two pins had a signal of +12V. The +3.3V rails are associated with memory. The +5V rails are typically used by the digital electronic components and circuits in the system. The +12V rails are used by disk drive motors and cooling fans~\cite{PowerSupplyArticle}.}

%{\color{magenta} Several challenges were encountered with this setup. First, we were obtaining only the voltages on the pins. Since we required power, we needed an additional 11 channels to collect current on the pins. The 22 channels of input exceeded the 16-channels available on our DAQ.  We temporarily acquired a second DAQ to solve the first challenge, but then encountered the second challenge of trying to unify the data for each voltage level across the 22 sources and to tease out meaning from the large set of data.  We found alternate solutions to these challenges.

%To address the first challenge, we tested several alternative options and eventually settled on using a compact DC voltage and current sensing PCB with analog output. The voltage and current sensing PCB determines the DC current by measuring the voltage drop across a shunt resistor, and then converts that measurement to analog voltage output that can be read by the DAQ. In addition to the rails that we were monitoring on the ATX power extender cable, we added two additional +12V rails that power the CPU, which led to monitoring a total of 13 voltage channels and 13 current channels.

%To address the second challenge (reduce the number of channels that we were monitoring), we noticed that the wires from the same voltage value were soldered together on the same contact point on the power supply. By grouping the rails by their voltage value, we ended up monitoring a total of four voltage channels and four current channels. This simplification meant that we no longer had to sum the currents from several different channels of input and also eliminated the need for the second DAQ. }

The vendor-provided DAQ software, TracerDAQ Pro  v. 2.3.1.0,
% provided by Measurement Computing with our DAQ for virtual instrumentation,
acquires, analyzes, and displays data from the DAQ's channels~\cite{TracerDAQPro}.
Our experimentation revealed that TracerDAQ Pro admits too little control over sampling rates and experiment length, and that acquired data precision is limited to three decimal places.
Consequently, we developed our own program that directly accesses the DAQ to gather data using custom software that had three distinct advantages: (1) data has 16 bits of precision; %directly accessed from the DAQ has nine decimal places; %which enabled us to observe much smaller variations.
(2) we were able to better control the sample recording rates and vary the sample timings; (3) we could make real-time calculations that helped assure that data is in the expected time ranges. %thus eliminating recording experiments when something was wrong.
%Fig.~\ref{fig:HW}(left) shows the voltage and current sense PCB  used on the hardware configuration to collect the power consumption of the general-purpose computer.
%Fig.~\ref{fig:HW}(right) shows the DAQ and power supply wiring harness used in our experiments.
% Code for Fig.s 1 and 2


As most malware initiates malicious traffic (e.g., click fraud, beaconing, spamming, etc.), unfiltered Internet  access for the experimental machine is necessary so malware operates with full functionality. For our experiments, an unfiltered, segregated network was created using a cellular data connection to the Internet that passed through another computer, the data repository, that was used to monitor and collect the power data before connecting to the experimental machine.
Two advantages emerged from this segregated network. (1) This design allowed the rootkits to behave normally, while avoiding any possibility of them infecting other computers on our network. (2) It allowed us to monitor, record, and analyze the experimental machine's network traffic.
For example, using Wireshark, we observed that several rootkits used in our experiments redirected web traffic to advertisement sites and malware as it attempted command and control contact.
% \begin{wrapfigure}{r}{.28\textwidth}
\begin{figure}
  \begin{minipage}[b]{0.46\linewidth}
  \centering
    \includegraphics[width=\textwidth,height=1.3in]{PCB6.png}
    %\caption{Power PCB sensor}
  \end{minipage}
  ~\hfill~
  \begin{minipage}[b]{0.46\linewidth}
    \centering
      \includegraphics[width=\textwidth,height=1.3in]{ATX_DAQ_ThirdConfiguration4.png}
      %\caption{Hardware configuration}
  \end{minipage}
  \caption{(Left) voltage and current sensor PCB depicted used to obtain the monitor power consumption from the experimental machine.
  (Right) ATX power extender cable attached to the DAQ depicted. The outputs for current, voltage, and ground from the sensor were wired to channels on the DAQ. %The DAQ is designed such that two input channels share a single ground.
  }
  \label{fig:HW}
% \end{wrapfigure}
\end{figure}



\subsection{Data Collection \& Rootkits}
\label{sec:data}
\begin{figure*}[!ht]
% \begin{wrapfigure}{r}[.7\textwidth}
\includegraphics[width=\textwidth]{SequenceOfEvents_4.png}
\centering
\caption{Power profile of +12V CPU depicted for each task before and after infection with Xpaj rootkit. Tasks labeled and demarcated by red vertical bars.}
\label{fig:SeqOfEvents}
% \end{wrapfigure}
\end{figure*}
% A separate machine, called the data repository, was used to monitor and collect the power data from the DAQ.
% This prevents detection and interference by malware on the experimental machine.
% The collected data was saved as a comma separated values (CSV) file in the data repository.
Although we collected data from eight channels (four voltage channels and four corresponding current channels), the results in this paper only utilize the +12V CPU rail's data.
% The difference between the +12V rails on the motherboard and the +12V CPU rail is that the +12V rails on the motherboard are used to power disk drive motors and fans, while the +12V CPU rail powers the CPU of the machine.
As part of the data preprocessing, the voltage and current channels were multiplied to obtain a quadruple %four-tuple
of power consumption for each sample time.
The sampling rate, computed as the median difference in power samples, was 0.0170s, with variance on the order of $10^{-6}$s. %Fig.~\ref{fig:expDesignFlowchart} shows the data collection workflow for our experiments.
 %CODE FOR DATA COLLECTION WORK FLOW DIAGRAM
% \begin{wrapfigure}{l}{.4\textwidth}
 %   \includegraphics[scale=0.40]{ExperimentalDesignFlowchart3}
  %  \centering
   % \caption{Data collection workflow}
    %\label{fig:expDesignFlowchart}
%\end{wrapfigure}

The power consumption of the general-purpose computer was recorded while completing the idle, IE, and registry tasks, first in a clean state and again after infection. % with a particular rootkit.
No other workload ran on the experimental machine.
To automate the tasks and ensure repeatability between experiments, a Python script orchestrated the following specified sequence of events.
During the data collection process, the experimental machine was idle for a three minute period.
In the case of IE, fifteen windows were open with a five second delay between each, and then each of these windows was closed before the script continued with the next task, probing the registry.
In case of probing the registry, we used regedit to copy all the information from the Windows registry to a .reg file.
By scripting workflow tasks, we ensure a repeatable sequence of commands.
To delimit and identify tasks in the power profile, a  C++ program was written and called between each task in order to insert ``markers'' that could be recorded by the DAQ.
This program performed calculations stressing the CPU of the experimental machine to 100\%, causing a noticeable plateau in the CPU power profile.
After data collection, a MATLAB script processed the power profile data, detected these embedded markers as start and end points to distinguish between different tasks of the experiment.
This is the source of the data segments used in the malware detection algorithms presented in this paper.

To ensure the experimental machine was returned to the same initial state between experiments, we made a clean installation of Windows using Clonezilla (\url{www.clonezilla.org/}). %~\cite{235}.
%{\color{magenta} Clonezilla is a partition and disk imaging/cloning program which we used to create an exact copy of the master hard drive. The image of the master hard drive was copied back to the experimental machine's hard drive between each experiment. Our original design used separate clean drives and infected drives, so that we could switch them out faster between experiments. Even though the drives were identical, differences appeared in the data because the hard drives consumed slightly different amounts of power. To eliminate this false signal, we now use a single drive for a complete experiment beginning with the clean image of Windows and then infecting it.}
With this preparation, the Python script was started on the experimental machine, while power consumption data was recorded on the data repository.
After completing the sequence of tasks in this uninfected state, the experimental machine was infected with a particular rootkit.
Then the sequence of tasks was repeated by the Python script and, after collection, the power consumption data was labeled as infected.
Fig. \ref{fig:SeqOfEvents} shows  power data for the +12V CPU rail from a single run of the Python script.
% In this run we first collected the power during each of the three tasks in an uninfected state, then infected the machine with the Xpaj rootkit and ran the same tasks again to collect power consumption data while infected.

As seen in Fig. \ref{fig:SeqOfEvents}, even within the sections where the machine is idle, there are still periods of elevated power use.
We investigated these events by correlating elevated power use events to Windows processes starting and ending.
We were able to attribute these power use events to Microsoft-provided background services which are a normal part of the Windows environment.
This illustrates the main challenge of profiling power consumption of fixed tasks %power-based malware detection
on a general-purpose computer, background processes contribute noise to the power profiles.
The hypothesis under investigation is that the executions of malware during various tasks and idle periods produce a significant-enough change in the power usage to admit accurate detection in the presence of the ambient but somewhat unpredictable normal executions.


%%% If space is needed, we split the column where the workflow picture resides using the maneuver below:
%The power consumption of the general-purpose computer was collected in two different scenarios, normal behavior (no\\
%\begin{minipage}{0.4\linewidth}
%\noindent rootkit running on the system) and malicious behavior (a rootkit was running on the system).
%For the data collection workflow, we assumed a clean installation of Windows, then power data was collected and labeled as normal. Subsequently, the experimental machine was infected and power data was collected and labeled as malicious. Fig.~\ref{fig:expDesignFlowchart} shows the data collection workflow for our experiments.\\
%\phantom{....}To ensure we had a clean installation of Windows 7, we used a tool called \textit{Clonezilla}~\cite{235}.
%Clonezilla is a partition
%\end{minipage}
%\begin{minipage}{.2\linewidth}
%\phantom{blah}
%\end{minipage}
%\begin{minipage}{.4\linewidth}
%	\phantom{aaa\\}
%    %CODE FOR EXPERIMENTSETUP FLOWCHART
%    \begin{figure}[H]
%    \includegraphics[scale=0.40]{ExperimentalDesignFlowchart}
%    \centering
%    \caption{Data collection workflow}
%    \label{fig:expDesignFlowchart}
%    \end{figure}
%	\phantom{blah\\}
%\end{minipage}\\
%\noindent and disk  imaging/cloning program that was used to create an exact copy of the master hard drive, and this hard drive was not exposed at all. {\color{BlueViolet} What does "not exposed at all " mean? Suggest rewording}

% \subsection{Rootkits}
% \label{sec:rootkits}
Next we discuss the rootkit samples used.
A rootkit is a ``kit'' consisting of small programs that allow a permanent or consistent, undetectable presence on a computer~\cite{Hoglund08}.
%that allow an attacker to gain control over a computer system without being detected
%escalate to maximum privileges
Basically, a rootkit locates and modifies the software on the computer system
%software  {\color{blue} what software??}
with the purpose of masking its behavior; for example, patching, a technique that modifies the data bytes encoded in an executable code, is an example of a type of modification that can be made~\cite{Hoglund08}.
%Attackers can install rootkits once they have obtained root or administrative access to the system. %{\color{magenta} Obtaining administrative access to the system can happen, for example, by exploiting a known vulnerability or a successful password attack.}
% An attacker with root privileges over a system can modify software, including software that might be used to detect malware.

For our experiments, five different malware programs were used, and
%, namely, \textit{Alureon}, \textit{Pihar}, \textit{Xpaj}, \textit{Sirefef} and \textit{Max Rootkit}.
each exhibits traits of a rootkit and/or actions for camouflaging itself.
% For example  that each one of these malware programs have to go to the registry in order to modify specific keys.
Alureon, also known as TDL4 or TDSS, is a Trojan that attempts to steal personal data.
% by affecting network traffic.
It encrypts itself in the master boot record, which makes it exceptionally hard to detect~\cite{ref:alureon1}, can remove competitor's malware, and hides communication via encryption. %Once Alureon is installed, it searches the system for any competitor's malware and removes it. %{\color{magenta}It also uses an encryption algorithm to hide its communications from traffic analysis tools that are sometimes used to detect suspicious transmissions~\cite{ref:alureon1}.}
% A variant of this rootkit is a Trojan called Pihar.
Pihar, an Alueron variant also known as Purple Haze, is capable of changing system settings without any manual direction, reconfiguring the Windows registry editor or keys, and disabling the AV software~\cite{ref:Pihar1}.
% Its rootkit capabilities include disabling the AV software to maintain itself hidden.
Like Alureon and Pihar, Xpaj is another rootkit that hides in the master boot record~\cite{ref:Xpaj1}. %, ref:Xpaj2, ref:Xpaj3}. % of the general-purpose computer.
% Xpaj is a botnet virus
%that usually infects computers via spam email messages that contain links to its download~\cite{ref:Xpaj1}.
% Another way of infection is via a Trojan dropper or when browsing web pages with hidden codes.
%Xpaj
Xpaj uses several methods of code obfuscation and encryption to hide its presence in the infected file.
%, and is able to connect to a command and control server to receive further instructions as part of a botnet~\cite{ref:Xpaj2}.
On the other hand, Sirefef, also known as Zero Access, is a trojan that is used to download other malware on the infected machine from a botnet that is mostly involved in bitcoin mining and click fraud.
Sirefef also overrides the registry and browser settings to hide itself~\cite{ref:ZeroAccess1}.
Like Alureon, it will spoof online search queries and the user will be redirected to malicious websites.
%Another rootkit that shares similar characteristics to Sirefef and Alureon is the Max rootkit.
Finally, Max rootkit is a Trojan that sometimes destroys information and files on its host computer, and changes Windows Explorer settings to download other malicious files~\cite{ref:MaxRootkit1}.%, ref:MaxRootkit2}.
% Like Alureon and Sirefef, it can change Windows Explorer settings to download other malicious files from external servers~\cite{ref:MaxRootkit1}.


Upon installation, to verify that the experimental machine was successfully infected with each one of these rootkit examples, two malware removal tools (TDSSkiller~\cite{ref:TDSSkiller} and Microsoft Windows Malicious Software Removal Tool~\cite{ref:WindowsRootkitRemovalTool}) were used.  % for detection purposes.
 Note that these tools were not used to clean the experimental machine.
We analyzed each rootkit using the web-based application called VxStream  Sandbox~\cite{ref:VxStreamSandbox}
%\footnote{\url{https://www.hybrid-analysis.com/} VxStream Sandbox is an automated malware analysis system that generates a behavioral report of the submitted malware. }
%More information of the features in VxStream Sandbox can be found in~\cite{ref:VxStreamSandbox}.
%We used this analysis of the five samples
 to see which Windows API functions were being called.
% In addition to verifying the rootkits were indeed successfully installed,
% Our analysis revealed in particular we analyzed rootkit actions, in particular, learning that each manipulates the Windows registry.
%Comparing these reports led us to include the copy of the Windows registry in the list of tasks, because several of the rootkits were manipulating the registry.
In total, for each of the three tasks (Idle, IE, and Registry) we collected power profile data for 15 runs in an uninfected state and 15 in an infected state (three per rootkit).


%{\color{Magenta}To verify that the experimental machine was successfully infected with a rootkit, tools such as OS Forensics, and Process Explorer were used. Note that the findings described here belong only to the Alureon rootkit.

%OS Forensics was used to establish a drive signature comparison prior to infection with the drive signature after the machine was infected. Results showed there was a difference between the two signatures. When using Process Explorer we noticed that new processes were appearing and disappearing after the experimental machine was infected. Interestingly, these processes belonged to Internet Explorer. To understand this behavior we used Wireshark to collect the network traffic and from the domains that were captured, one of them got our attention (term015ter12.com). Several websites had this domain registered as malicious~\cite{DomainBlocklist} After all these analyses, we strongly believe that the experimental machine was successfully infected.}


==> 4.1-features-2.tex <==

\subsection{Features}
\label{sec:features}
Modeling diverse qualities of the data gives more avenues of detection; hence, we craft a variety of features modeling statistical properties of the power data sample as well as many time-varying characteristics.
For each task (IE, Registry, Idle), the power profile of a given run is transformed into a feature vector.
The first four features are statistical moments, which encode characteristics of the power data regarded as a set of independent and identically distributed (IID) samples of a distribution.
The remaining features ($L^2$ distance, permutation entropy, and Data Smashing distances) seek to describe time-dependent properties of the power profile.
For these features it is convenient to have uniformly sampled power data.
To obtain uniform times, all observations in a run are shifted by their initial time, so time uniformly begins at $t=0$.
Next, the time-stamped data points are linearly connected to define the power profile for all time values, and then sampled for each multiple of $.01$ seconds.
Note power samples occur with a median $.0170$ seconds apart and variance on the order of $10^{-6}$ seconds, so by using the finer-grained samples, we obtain a close approximation of the observed profile that is also uniformly spaced.
% Below we describe each of the features in detail.

\subsubsection{Statistical Moments}
\label{sec:moments}
In order to model the distribution of the power data, we use (empirical estimates of) the mean (first moment), variance, skewness, and kurtosis (second-fourth normalized central moments).\footnote{Kurtosis $:=  \sum_{i = 1}^N (x_i - \mu)^4/(N\sigma^4) - 3.$ This follows Fisher's definition, with 3 subtracted so normally distributed data yield 0.}
% For a given run of a task let $(x_i : i = 1,\dots, N) $ denote the power observations (in any order).
%Then the moments above have the following definitions:\footnote{Note that alternate definitions exist to adjust for bias in the estimator.}
% \begin{itemize}
%     \item Mean, denoted $\mu := \sum_{i=1}^N x_i/N$.
%     \item Variance, denoted $\sigma^2 := \sum_{i=1}^N (x_i - \mu)^2/N$. (Note that $\sigma$ denotes the standard deviation).
%     \item Skewness $:= \sum_{i=1}^N (x_i - \mu)^3/(N\sigma^3).$
%     \item Kurtosis $:=  \sum_{i = 1}^N (x_i - \mu)^4/(N\sigma^4) - 3.$ This follows Fisher's definition, with 3 subtracted so normally distributed data yield 0.
% \end{itemize}
% Roughly speaking,
% mean gives the average value of the data, variance measures how spread the data is,
% skewness indicates if more of the data is left/right of the mean, and kurtosis measures of how much of the data lies in the tails.
% For each task, each of the moments above are computed making the first four features.

\begin{figure*}
    \includegraphics[scale=0.5]{baseline-functions.png}
    \centering
    \caption{(Watts vs. Seconds) Canonical profiles (baselines for $L^2$ error) per task found by clustering unsupervised training data (ten uninfected runs) with $k$-means clustering with $L^2$ distance. Gap statistic used to find the no. of clusters, $k$, and $k = 1$ (as expected) is found in each case. Centriods (means of each cluster) depicted.
    %This indicates that all ten runs were close in an $L^2$ sense.
    %Centroids of the clusters depicted and used as the baseline profile for computing $L^2$ error feature. Note that the time span ($x$-axis) is not uniform across the three plots.
    }
    \label{fig:centroids}
\end{figure*}
\subsubsection{$L^2$-Norm Error}
\label{sec:l2}
Regarding each power profile as a function $p(t)$, the $L^2$ norm (defined as $[ \int |p|^2 dt]^{1/2}$)  furnishes a natural (Euclidean) distance for pairwise comparison.
As we have constructed uniformly sampled approximations of the profiles, multiplying the usual ($l^2$ Euclidean) vector distance to the tuple of power observations by the $\Delta t = .01$ gives a close approximation to the integral.
To construct baseline profile, we cluster the uninfected training data using $k-$means clustering, with $k$ determined by the gap statistic method~\cite{tibshirani2001estimating}.
This provides a sanity check\textemdash we hypothesize that our uninfected training runs should be similar; hence, we expect a single cluster with the centroid a canonical ``baseline'' function.
Indeed, for all tasks a single canonical baseline was found by the gap statistic method.
%, except the notepad task for, which two clusters were found.
Fig.~\ref{fig:centroids} depicts the baselines for each task, as found on the ten uninfected training runs used for unsupervised training.
For the supervised approach, the baseline is created from the 12 clean training profiles.
Finally, the feature for a given profile is the $L^2$ distance to the baseline.


\subsubsection{Permutation Entropy}
\label{sec:pe}
Permutation Entropy, is a method of time-series analysis that detects deviations in the short-term wiggliness (roughly speaking) and has been used in various time-series detection applications including  epilepsy~\cite{cao2004detecting} and motor bearing fault detection~\cite{zhang2015novel}.
Our formulation follows Cao et al.~\cite{cao2004detecting}.
From a time-series data vector, $(x_1, \dots, x_N)$ (a power profile in our case) fix an $m$-length contiguous sub-vector $(x_i, x_{i+1}, ..., x_{i+m-1})$ and denote this vector as $(y_0, ..., y_{m-1})$.
Next sort the elements into increasing order, $(y_{j_0}, ..., y_{j_{m-1}})$, so either $y_{j_k} < y_{j_{k+1}}$  or $y_{j_k} = y_{j_{k+1}}$ and $j_k + 1$ = $j_{k+1}$.
Now, $(j_0, ..., j_{m-1})$ is the permutation of the numbers $(0, 1,..., m-1)$ indicating the rearrangement necessary to sort the $m$-length vector.
Given a time-series data vector $(x_1, \dots, x_n)$ (a power profile), we extract contiguous sub-vectors of length $m$ with overlap $m/2$, i.e., $(x_1, ..., x_m)$, $(x_{\frac{m}{2}+1}, ... , x_{m + \frac{m}{2}}), $ etc.
Each $m$-length vector is converted to one of the $m!$ permutations by the process above, and we represent the time-series as a bag of permutations.
Our goal is to learn how rare/likely the profile is by understanding the likelihood of its permutations.
To do this, we require a probability distribution over the sample space of $m!$ permutations.

For a fixed task, we estimate the needed probability distribution from the training runs on that task.
Let $\mathcal{O}$ be the observations (multiset) of permutations across all training runs, and for each permutation $\gamma = (j_0, ..., j_{m-1})$,
let $\#( \gamma , \mathcal{O} )$ denote the number of times $\gamma$ is observed in $\mathcal{O}$.
Then we use the maximum a posteriori (MAP) estimation with uniform prior to estimate $\gamma$'s probability,
% $$P( \gamma ) := \frac{\#( \gamma, \mathcal{O} ) +1 }{ |\mathcal{O}|+m!}.$$
$P( \gamma ) :=  (\#( \gamma, \mathcal{O} ) +1)/(|\mathcal{O}|+m!).$
%
This allows permutations never observed in training to have positive likelihood, albeit very small.
It is clear from the MAP estimate that $m$ must be chosen carefully, as for moderate values of $m$, $m!$ will easily dominate $|\mathcal{O}|$, washing out the contribution of our observations.
We chose $m = 6$, which gives $m! = 720$, while $|\mathcal{O}|$ = 61,680 for IE, 6,240 for Registry, and 53,980 for Idle tasks.
Finally, for a given run we will compute the entropy of the observed permutations as IID samples from the distribution above.
After converting an observed power profile to a bag of permutations, $(\gamma_i: i = i, ..., n )$, we compute the permutation entropy, that is, the expected information of the permutation,
$\hat{H} = (1/n) \sum_i -\log(P(\gamma_i))P( \gamma_i ).$

\subsubsection{Data Smashing Distances}
\label{sec:dsd}
Data Smashing distance (DSD) is a new algorithm pioneered by Chattopadhyay and  Lipson~\cite{ chattopadhyay2014data} %chattopadhyay2013abductive,
for quantifying the distance between two time-varying sequences.
DSD assumes the non-restrictive hypothesis that each sequence is a sample from a probabilistic finite state automata (PFSA) and approximates the distance between the underlying PFSAs.\footnote{A PFSA is (roughly speaking) a generative model for sampling a sequence of symbols and is composed of a set of states, a stochastic state transition matrix, and rules giving fixed symbol emissions on the transitions. PFSA are similar to, but conceptually simpler than, hidden markov models (HMMs). HMMs emit a sequence of symbols in a two-step process. The new state is sampled according to the transition probabilities. Then a symbol is sampled from the emission distribution for the new state. Rather than a probabilistic symbol emission depending on the state, PFSA emit a fixed symbol determined by the transition.}
Roughly speaking, PFSA are applicable models to any sequence of symbols where the probability of a current symbol depends only on the previous symbols.
The DSD algorithm relies on mathematical developments involving PFSA by Wen and Ray~\cite{wen2012vector} who discover a groups structure and metric on the set of PFSA. %which we only briefly discuss.
%Wen and Ray's work develops a group structure and metric (distance function) on the set of PFSA.
DSD gives a novel, computationally efficient algorithm for approximating the distance between two PFSA from sufficiently long symbol strings sampled from each.
This operationalizes the developments of Wen and Ray, as one need not know nor try to infer the PFSA from the symbol observations.

In order to apply DSD, users must transform their time-varying data into a sequence of symbols that is sufficiently long.
The expected string length required by the DSD algorithm is strictly increasing in the number of symbols (factorial in this variable) and the product of the symbol probabilities.\footnote{For details see the Proposition 13 in the supplementary text of% Chattopadhyay and Lipson
~\cite{chattopadhyay2014data}.}
Although the desired PFSA distance is symmetric ($d(s1, s2) = d(s2, s1)$), DSD uses a probabilistic algorithm to approximate the distance, and will produce similar but, in general, not identical values as the order is switched.
For this reason, given two strings $s_1$ and $s_2$, we compute $d(s1, s2)$ and $d(s2, s1)$ and store the average of the two as the distance.
If either distance is not returned, it indicates our strings are not long enough, and this feature is not used.
% Insufficient length occurs in our application only for the Idle task when using the shape sequences.


We employ DSD on two symbol representations of the power data, separately.
The first transforms power samples into two symbols, ``high'' and ``low'', and is a stereotypical application of Data Smashing.
This is referred to hereafter as ``DSD Data Distance.''
The threshold for the binary representation is chosen for each pair of profiles, so the number of power readings over and under the threshold are equal.
This maximizes the product of the probabilities of each symbol, which helps ensure the symbols are sufficiently long.
Note that the baseline observed profiles are fixed, and to compute the DSD Data Distance between the baseline and a newly observed given test profile, the threshold for encoding both profiles as a binary high/low sequence is dependent on both profiles.
Hence, the binary sequence for the baseline profile will be slightly different in each comparison, but no prior knowledge of any test data is necessary.
\begin{figure}
    \includegraphics[scale=0.23]{shapes.png}
    \centering
    \caption{(Watts vs. Seconds) Canonical shapes found by clustering three-second intervals of training data. Note that the four shapes characterize {\color{red}high power}, {\color{blue} low power}, {\color{darkolivegreen}  falling power}, and {\color{teal} rising power}. }
    %\color{OliveGreen}
    \label{fig:shapes}
\end{figure}


The second application seeks to model sequences of shapes in the power curves and is referred to as ``DSD Shape Distance.''
To produce the shapes, the training profiles are cut into three-second intervals with 1.5-second overlap.
Then the bag of all three second snippets are clustered using $k$-means and $L^2$ distance as in Sec.~\ref{sec:l2}.
We manually investigated the centroids as $k$ varied, choosing $k=4$ as is maximal for which the centroids are not very similar curves.
See Fig.~\ref{fig:shapes} depicting the four canonical shapes learned from the data.
Finally, given a power profile, we cut it into a sequence of three-second intervals, overlapping by 1.5 seconds, and assign to each interval
the closest canonical shape.
This transforms a power profile into a sequence of four ``shape'' symbols.
Our conjecture is that profiles that exhibit a clear pattern when uninfected (e.g., the IE baseline, top Fig.~\ref{fig:centroids}), will give a regular sequence of shapes that may be disrupted by malware execution.

In both transformations to a sequence of symbols, every sequence is concatenated with itself 100 times to ensure the strings are long enough to perform the algorithm.
This can be conceptualized as a simulation of running the same task repeatedly 100 times.
DSD Shape distance is not applicable to the the Idle task runs because the strings are not long enough.
This is likely caused by the fact that the flat, low power shape dominates the probabilities, making the product of the four symbols probabilities very small.
To obtain both the DSD Data and DSD Shape feature value for a given a power profile, we compute the distance between its symbol sequence and that of all ten training runs concatenated together.



% DS distances
% 	Shape distance
% 	1. cannonical shapes To get the shapes, we cut each training run into 3 second intervals, overlapping by 1.5 s. Then cluster all the pieces w/ k-means adn l2 distance. We manually chose that max number of cluster centers that weren't too close together. (after 4 they got really close together. )
% 	2. Given a run, cut it into the 3 second, intervals and preserve order.  Each piece is represented by the cluster it is a member of. This transforms a power curve into a sequence of the 4 canonical shapes.
% 	3. Baseline string: Concatenate the 10 training samples 100 times to get a long enough string of symbols (look up this detail)
% 	4. for each run, switch to symbol sequence and apply DS distance against the baseline.
% 	NEED to include plots of the canonical shapes.

% 	Data distance
% 	1. We take the run in question and the baseline function (found from clustering for the L2 distance) and find the threshold for which # power readings over the threshold and # under are about equal (maximize entropy of states across the union of the power readings in both runs).
% 	2. both the run and the baseline run are converted to a 2-symbol sequence (high if over, low if under the threshold).
% 	3 apply DS distance after concatenating each of them to themselves 100 times.

% 	In both the final distance is (eps12 + eps21)/2.


% Permutation entropy z-score:
% 	Inputs:
% 		- m = 6 (len of a piece we will consider)
% 		- the training runs (for now fix the task and the rail)
% 	Algorithm:
% 		1. get a probability of permutations observed in all the training data
% 			- cut each run into len m pieces and let them overlap by m/2. (so we have [x1, x2, ..., x_n] --> [ [ x_1, .., x_6 ] [x4, .., x10] , ... ])
% 			- define permutation (piece) = rearrangement of indices that sorts them (e.g. sorted(x1, x2, x3, .., x6) = (x3, x1, x6, x2, x4, x5) then permutation (piece ) = (3,1,6,2,4))
% 			- let data = [ permutation(pieces) for pieces in any run ]
% 			- set p(permutation) = (count(permutation in data) + 1 ) / m!
% 				- hence, we can't have m too big or the prior washes out the observations (m! is just too much)
% 				- need to count the len(data) and see how much it was and compare to m! so i can show why we chose 6.
% 		2. get the mean and variance of information of permutations in the training data
% 			- now we compute entropy : = expected information = E(-log(p(x))) = sum p(x)*-log(p(x))  = H
% 			- and we compute information variance = E(log(p(x))^2) - H^2
% 		3. given a new run
% 			- cut into pieces and switch pieces to permutations so we have [y1, y2, .. yN]
% 			- empirical mean of information = (1/N) sum (p(yj)*-log(pj))
% 			- compute z-score |emperical mean - H|/var^.5
% 			- flag if z > 1


% Threshold notes:
% 	For every feature we compute a z_score. z_score >=1 gets a vote from that detection method  b/c it's value is at least 1 standard deviation from the mean.

%     For each task (Internet Explorer, Registry, Idle, and Notepad), the statistics above are computed for each run (training and testing).
% Next, rather than using the raw statistics, we normalize these features by computing a z-score from the training runs statistics.
% Specifically,  computing the mean and variance of the observed training statistics (
% Basic statistics z-score:
% 	stats considered: moment:  1 (mean), 2 (variance), 3 (skewness), 4 (kurtosis) and also runtime.
% 	1. For each we run (fix the task and the rail) we compute the stat
% 	2. let m = mean (stat over the training runs), and v = variance of the statistic over the training runs
% 	3. for a test run, compute the statistic, s and compute z= |s-m|/sqrt(v)
% 	4. flag if z > 1


% 	Finally, how many votes to be flagged as malware? we look at the training data and take the mean number of votes + the standard deviation:

% 	mean number of votes for training on task notepad = 3.7
% 	variance of number of votes for training on task notepad = 1.21
% 	threshold for task notepad = 4.8

% 	mean number of votes for training on task idle = 4.0
% 	variance of number of votes for training on task idle = 1.2
% 	threshold for task idle = 5.09544511501

% 	mean number of votes for training on task ie = 3.3
% 	variance of number of votes for training on task ie = 2.61
% 	threshold for task ie = 4.91554944214

% 	mean number of votes for training on task registry = 4.2
% 	variance of number of votes for training on task registry = 1.36
% 	threshold for task registry = 5.36619037897

